Performance Evaluation of Dynamic Metasurface Antennas: Impact of Insertion Losses and Coupling

This paper evaluates the performance of multi-user massive multiple-input multiple-output (MIMO) systems in which the base station is equipped with a dynamic metasurface antenna (DMA). Due to the physical implementation of DMAs, conventional models widely-used in MIMO are no longer valid, and electromagnetic phenomena such as mutual coupling, insertion losses and reflections inside the waveguides need to be considered. Hence, starting from a recently proposed electromagnetic model for DMAs, we formulate a zero-forcing optimization problem, yielding an unconstrained objective function with known gradient. The performance is compared with that of full-digital and hybrid massive MIMO, focusing on the impact of insertion losses and mutual coupling.

==> setup/preamble.tex <==
\IEEEoverridecommandlockouts % Comment this out if no funding/thanks.

\makeatletter
\let\NAT@parse\undefined
\makeatother

% Packages
\usepackage{amsmath,amssymb,amsfonts,amsthm,commath,esint}
\usepackage[numbers,sort&compress]{natbib}
\renewcommand{\bibfont}{\footnotesize}
\usepackage{mathtools}
\usepackage{glossaries}
\usepackage{color}
\usepackage{multirow}
\usepackage{enumitem}
\usepackage{physics}
\usepackage{optidef}
\usepackage{mleftright}
\usepackage{cuted}
\usepackage[linesnumbered]{algorithm2e}
\usepackage{algpseudocode}
\usepackage{microtype}
\usepackage{bm}
\usepackage{siunitx}

\SetKwInput{kwInit}{Initialization}

% IEEE recomended option for subfigures -> Do not use subcaption package
\ifCLASSOPTIONcompsoc
    \usepackage[caption=false, font=normalsize, labelfont=sf, textfont=sf]{subfig}
\else
\usepackage[caption=false, font=footnotesize]{subfig}
\fi

% Footnote definition 
\makeatletter
\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}
\makeatother

% Acronyms
\newacronym{MIMO}{MIMO}{multiple-input multiple-output}
\newacronym{mMIMO}{mMIMO}{massive \gls{MIMO}}
\newacronym{BS}{BS}{base station}
\newacronym{FD}{FD}{full-digital}
\newacronym{UE}{UE}{user equipment}
\newacronym{RF}{RF}{radio-frequency}
\newacronym{SNR}{SNR}{signal-to-noise ratio}
\newacronym{SINR}{SINR}{signal-to-interference-plus-noise ratio}
\newacronym{PEC}{PEC}{perfect electric conductor}
\newacronym{DMA}{DMA}{dynamic metasurface antenna}

% Easier sine and cosine
\newcommand{\es}[1]{\sin{\left(#1\right)}}
\newcommand{\ec}[1]{\cos{\left(#1\right)}}
\newcommand{\p}[1]{\left(#1\right)}


% Vector and matrix typesetting command
\renewcommand{\vec}[1]{\mathbf{\lowercase{#1}}}
\newcommand{\nvec}[1]{\hat{\mathbf{\lowercase{#1}}}}
\newcommand{\mat}[1]{\mathbf{\uppercase{#1}}}

% More compact integral
\newcommand{\Int}{\int\limits}

% Partial derivative
\newcommand{\der}[2]{\frac{\partial \,#1}{\partial \,#2}}

% Trace
%\newcommand{\tra}[1]{\text{Tr}\left\{#1\right\}}

% Exponentials
\renewcommand{\exp}[1]{\mathrm{exp}{\left(#1\right)}}
\newcommand{\e}[1]{\mathrm{e}^{#1}}

% Since function
\DeclareMathOperator{\sinc}{sinc}

% USE \evalat*{}{} for auto size adjustment, \evalat[\bigg]{}{} for manual size adjustment
% https://tex.stackexchange.com/a/294528
\NewDocumentCommand{\evalat}{sO{\big}mm}{%
  \IfBooleanTF{#1}
  {\mleft. #3 \mright|_{#4}}
  {#3#2|_{#4}}%
}

% Provides interface for expectition and given  e.g. \Aver{K \given L}, for big use \Aver[\bigg]
\providecommand\given{}
\DeclarePairedDelimiterXPP\Aver[1]{\mathbb{E}}{[}{]}{}{
\renewcommand\given{  \nonscript\:
  \delimsize\vert
  \nonscript\:
  \mathopen{}
  \allowbreak}
#1
}

% Argmin and argmax
\DeclareMathOperator*{\argmin}{arg\,min} % thin space, limits underneath in displays
\DeclareMathOperator*{\argmax}{arg\,max} % thin space, limits underneath in displays
\DeclareMathOperator*{\diag}{diag} % thin

\DeclareMathOperator{\Si}{Si}

% Comments commands
\newcommand{\rjw}[1]{{\color{green}{\textit{{\footnotesize RJW:} {\footnotesize #1}}}}}
\newcommand{\jy}[1]{{\color{blue}{\textit{{\footnotesize JY:} {\footnotesize #1}}}}}
\newcommand{\pre}[1]{{\color{red}{\textit{{\footnotesize PRE:} {\footnotesize #1}}}}}
\newcommand{\edc}[1]{{\color{pink}{\textit{{\footnotesize EDC:} {\footnotesize #1}}}}}
